Gaze-supported Large Language Model Framework for Bi-directional Human-Robot Interaction

The rapid development of Large Language Models (LLMs) creates an exciting potential for flexible, general knowledge-driven Human-Robot Interaction (HRI) systems for assistive robots. Existing HRI systems demonstrate great progress in interpreting and following user instructions, action generation, and robot task solving. On the other hand, bi-directional, multi-modal, and context-aware support of the user in collaborative tasks still remains an open challenge. In this paper, we present a gaze- and speech-informed interface to the assistive robot, which is able to perceive the working environment from multiple vision inputs and support the dynamic user in their tasks. Our system is designed to be modular and transferable to adapt to diverse tasks and robots, and it is capable of real-time use of language-based interaction state representation and fast on board perception modules. Its development was supported by multiple public dissemination events, contributing important considerations for improved robustness and user experience. Furthermore, in two lab studies, we compare the performance and user ratings of our system with those of a traditional scripted HRI pipeline. Our findings indicate that an LLM-based approach enhances adaptability and marginally improves user engagement and task execution metrics but may produce redundant output, while a scripted pipeline is well suited for more straightforward tasks.

==> prompt.tex <==
\vspace{0.2cm}
\begin{figure}[t!]
\centering
\begin{tcolorbox}[colframe=black!75, colback=white, left=0mm, right=0mm, top=0mm, bottom=0mm, sharp corners]

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
    You are the brain of [...], a robot from [...]
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{1.} \\
    \scriptsize \textit{Setup description}
\end{minipage}
\end{tcolorbox}

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
Your input has the structure of a Python dictionary:

self.state\_description
= \{"transcription": \textless what the user said or asked\textgreater, "object\_ids":
\textless a list containing the object ids\textgreater, \\
"scene\_description": \textless a string contains the scene description\textgreater, \\
"object\_labels": \textless a list of objects in the scene\textgreater, \\
"fixated\_object\_label": \textless the label of the object that the user looked at\textgreater,
"fixated\_object\_id": \textless the id of the object that the user looked at\textgreater,
"object\_coordinates": \textless A list with 3d coordinates where the objects are according to your position\textgreater\}

[...]
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{2.} \\
    \scriptsize \textit{Input structure description}
\end{minipage}
\end{tcolorbox}

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
Your task is [...]. Let's think step by step.
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{3.} \\
    \scriptsize \textit{Task description and CoT prompting}
\end{minipage}
\end{tcolorbox}

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
These are the possible API function calls you can generate: \\
´´´python \\
\#activity.talker("\textless final\_output\_the\_robot\_talks\_to\_the\_user\textgreater") \\
\#activity.think\_step\_by\_step("\textless your\_inner\_monologue\textgreater") \\
\#activity.executor(\textless if [...]\textgreater) \\
\#activity.shaking\_head(\textless if\_you\_dont\_agree\textgreater) \\
\#activity.nodding(\textless If\_you\_agree\textgreater) \\
´´´python
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{4.} \\
    \scriptsize \textit{SDK connection}
\end{minipage}
\end{tcolorbox}

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
If you final answer contains a "Yes", then add activity.nodding(). If it contains a "no", then add activity.shaking\_head().

[...]
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{5.} \\
    \scriptsize \textit{Optional examples}
\end{minipage}
\end{tcolorbox}

\begin{tcolorbox}[left=-0.25mm, right=-0.25mm, top=-0.25mm, bottom=-0.25mm, boxrule=0mm, width=\linewidth, sharp corners]
\begin{minipage}{0.8\textwidth} % Left column (80% of width)
    \raggedright
    \scriptsize
Your possible output always looks like the following: \\
activity.think\_step\_by\_step(\textless your\_inner\_monologue\textgreater) \\
\textless Add activity.shaking\_head(), activity.nodding() or activity.executor() here if needed\textgreater \\
activity.talker(\textless final\_output\textgreater)

[...]
    \end{minipage}%
\hfill % Space between columns
\begin{minipage}{0.2\textwidth} % Right column (20% of width)
    \centering
    \textbf{6.} \\
    \scriptsize \textit{Output structure description}
\end{minipage}
\end{tcolorbox}

\end{tcolorbox}
\raggedright
\caption[The prompt of the reasoning module with a modular design.]{The prompt of the reasoning module with a modular design. \textbf{1)} Initial setup description \textbf{2)} Expected input structure in the form of a Python dictionary. \textbf{3)} Task description along with chain-of-thought prompting, guiding the module’s reasoning process \textbf{4)} Example for available SDK connections and API function calls that integrate the robot’s functionality \textbf{5)} Examples for generating actions (e.g., nodding or shaking head) \textbf{6)} Structured format of the final output.}
\label{abb:prompt}
% Very brief summary of what is described in the caption in the figures right in the numbers
\end{figure}
